Towards Graph Self-Supervised Learning with Contrastive Adjusted Zooming

Graph representation learning (GRL) is critical for graph-structured data analysis. However, most of the existing graph neural networks (GNNs) heavily rely on labeling information, which is normally expensive to obtain in the real world. Although some existing works aim to effectively learn graph representations in an unsupervised manner, they suffer from certain limitations, such as the heavy reliance on monotone contrastiveness and limited scalability. To overcome the aforementioned problems, we introduce a novel self-supervised graph representation learning algorithm via Graph Contrastive Adjusted Zooming, namely G-Zoom, to learn node representations by leveraging the proposed adjusted zooming scheme. Specifically, this mechanism enables G-Zoom to explore and extract self-supervision signals from a graph from multiple scales: micro (i.e., node-level), meso (i.e., neighborhood-level), and macro (i.e., subgraph-level). Firstly, we generate two augmented views of the input graph via two different graph augmentations. Then, we establish three different contrastiveness on the above three scales progressively, from node, neighboring, to subgraph level, where we maximize the agreement between graph representations across scales. While we can extract valuable clues from a given graph on the micro and macro perspectives, the neighboring-level contrastiveness offers G-Zoom the capability of a customizable option based on our adjusted zooming scheme to manually choose an optimal viewpoint that lies between the micro and macro perspectives to better understand the graph data. Additionally, to make our model scalable to large graphs, we employ a parallel graph diffusion approach to decouple model training from the graph size. We have conducted extensive experiments on real-world datasets, and the results demonstrate that our proposed model outperforms state-of-the-art methods consistently.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> bio.tex <==
\vspace{-1cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/yizhen.jpeg}}]{Yizhen Zheng} 
received the M.Bus.Info.Sys degree from Monash University, Melbourne, Australia, as Dux in 2020, M.Bus degree from Monash University in 2018 and B.B.A degree from Shenzhen University, Shenzhen, China, in 2016. He is a PhD student at Monash University. His research interests lie in data mining, machine learning, graph neural networks (GNNs) and graph representation learning (GRL).
\end{IEEEbiography}

\vspace{-1.5cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/mingjin.jpg}}]{Ming Jin} 
received the B.Eng. degree from the Hebei University of Technology, Tianjin, China, in 2017, and M.Inf.Tech. degree from the University of Melbourne, Melbourne, Australia, in 2019. 
He is currently pursuing his Ph.D. degree in computer science at Monash University, Melbourne, Australia.
His research focuses on graph neural networks (GNNs), time series analysis, data mining, and machine learning. 
\end{IEEEbiography}

\vspace{-1.5cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/shirui-bio.jpg}}]{Shirui Pan} received a Ph.D. in computer science from the University of Technology Sydney (UTS), Ultimo, NSW, Australia, in 2015. He is currently a Professor with the School of Information and Communication Technology, Griffith University, Australia. 
His research interests include data mining and machine learning. To date, Dr. Pan has published over 100 research papers in top-tier journals and conferences, including TPAMI, TNNLS, TKDE, ICML, and KDD. 
He is an awardee of a prestigious ARC Future Fellowship (2021-2025).
\end{IEEEbiography}

\vspace{-1.5cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/IT_Staff_0923.jpg}}]{Yuan-Fang Li} is an Associate Professor at Department of Data Science and Artificial Intelligence, Faculty of Information Technology, Monash University, Australia. He received his Ph.D.\ in computer science from National University of Singapore in 2006. His research interests include knowledge graphs, natural language processing and knowledge representation and reasoning.
\end{IEEEbiography}

\vspace{-1.5cm}
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/ph.png}}]
{Hao Peng} is currently an Assistant Professor at the Beijing Advanced Innovation Center for Big Data and Brain Computing in Beihang University. 
His research interests include representation learning, social network mining and reinforcement learning. To date, Dr Peng has published over 60 research papers in top-tier journals and conferences, including the IEEE TKDE, TC, TPDS, TITS, ACM TOIS, TKDD, TIST, and Web Conference.
\end{IEEEbiography}

\vspace{-1.5cm}
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/MingLi-bio.jpg}}]
{Ming Li} received the Ph.D. degree in 2017 from the Department
of Computer Science and IT, La Trobe
University, Melbourne, VIC, Australia.
%After that, he acted as a research officer at the
%Department of Mathematics and Statistics at La
%Trobe University, Melbourne, VIC, Australia. %He
%was also a Post-Doctoral Fellow with the Department of Information
%Technology in Education, South China Normal University, Guangzhou,
%China. 
He is currently a Distinguished Professor with
the Key Laboratory of Intelligent Education Technology and Application of Zhejiang Province, Zhejiang Normal University, Jinhua,
China. His current research interests include  graph neural networks, graph representation learning, etc. He is
an Action Editor of Neural Networks (Elsevier, 2022-2024). % He, as a leading guest editor, is currently
%organizing a special issue, i.e., “\emph{Deep Neural Networks for Graphs:
%Theory, Models, Algorithms and Applications}”, on IEEE TNNLS.
\end{IEEEbiography}

\vspace{-2cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/zhao-bio.png}}]{Zhao Li}
received the Ph.D. degree in computer science from the University of Vermont with the Excellent Graduate Award in 2012.  He is currently an adjunct professor with Zhejiang University, Alibaba-Zhejiang University Joint Institute of Frontier Technologies, Hangzhou, China. He is also the funder of Link2Do Technology Ltd., Hangzhou. He has published several papers in prestigious conferences and journals, including the World Wide Web Conference (WWW), the AAAI Conference on Artificial Intelligence (AAAI), IEEE International Conference on Data Engineering (ICDE), International Conference on Very Large Data Bases (VLDB), IEEE TRANSACTIONS ON KNOWLEDGE AND DATA ENGINEERING (TKDE), and so on. His research interest lies in reinforcement learning, big-data-driven security, and large-scale graph computing.
\end{IEEEbiography}
